SynthForge: Synthesizing High-Quality Face Dataset with Controllable 3D Generative Models

Recent advancements in generative models have unlocked the capabilities to render photo-realistic data in a controllable fashion. Trained on the real data, these generative models are capable of producing realistic samples with minimal to no domain gap, as compared to the traditional graphics rendering. However, using the data generated using such models for training downstream tasks remains under-explored, mainly due to the lack of 3D consistent annotations. Moreover, controllable generative models are learned from massive data and their latent space is often too vast to obtain meaningful sample distributions for downstream task with limited generation. To overcome these challenges, we extract 3D consistent annotations from an existing controllable generative model, making the data useful for downstream tasks. Our experiments show competitive performance against state-of-the-art models using only generated synthetic data, demonstrating potential for solving downstream tasks. Project page: https://synth-forge.github.io

==> sec/0_abstract.tex <==
\begin{abstract}
% Generative models have unlocked the potential of rendering photorealistic human face images, yet, their integration for training downstream tasks remains underexplored, mainly due to the lack of controllable annotations. 
% In this work, we leverage an existing generative model for synthesizing high-quality face images, while utilizing 3D Morphable Models (3DMMs) to extract 3D-aware annotations. 
% We synthesize dense multi-modal annotations and showcase the efficacy of generative synthetic data by training a multi-task model for facial analysis. 
% We further utilise a label fine-tuning strategy that refines the predictions from our synthetically trained multi-task network, facilitating its applicability for any real-world dataset. 
% At the core of our approach is a robust dense multi-modal training pipeline, enhanced with cross-task consistency and self-supervised losses. 
% Our experiments show competitive performance against state-of-the-art single and multi-task models. 
% We shall release of our synthetic dataset, pretrained models, and the accompanying codebase for the community to further explore the usage of synthetic data for real-world facial analysis tasks. 
% Through our approach, we take a step towards broader adoption of generative synthetic data in the computer vision domain.




% 

% \begin{enumerate}
% \item Controllable generative models are very powerful, they are learned from the real world distribution, hence avoid the uncanny valley issue of the traditional graphics rendering and the requirements of assets pool.
% \item We want to leverage controllable generative model as our synthetic data generation engine to create tons of image-gt pairs.
% \item However, while Controllable generative models are learned from massive data, their latent space is often too vast to obtain meaningful sample distributions for downstream task with limited generation. --> uniform sampling is not sufficient.
% \item We propose to forge the downstream task models together with the controllable generative data engine to make the data generation process steerable and optimized for the downstream task in an active learning way.
% \item This is in contrast from the previous paradigm of human-prior based data generation, where our generated data distribution is optimized for solving the specific discriminative task. Task-wise, similar to the DataComp paper from LAION, but we are building an active learning framework to achieve it instead of relying on crowd-source human effort to find the best task\&model-specific data generation/composition
% \end{enumerate}

Recent advancements in generative models have unlocked the capabilities to render photo-realistic data in a controllable fashion.
Trained on the real data, these generative models are capable of producing realistic samples with minimal to no domain gap, as compared to the traditional graphics rendering.
However, using the data generated using such models for training downstream tasks remains under-explored, mainly due to the lack of 3D consistent annotations.
Moreover, controllable generative models are learned from massive data and their latent space is often too vast to obtain meaningful sample distributions for downstream task with limited generation.
To overcome these challenges, we extract 3D consistent annotations from an existing controllable generative model, making the data useful for downstream tasks.
% We further propose integrating downstream task models with the controllable generative data engine to ensure steerable data generation and obtain meaningful task-specific sample distribution.
% This is in contrast from the traditional paradigm of generation wherein data distribution is decided using human-prior for the specific task.
% (consumption?).
% In this work, we leverage an existing controllable generative model for synthesizing high-quality facial images and extract 3D-consistent annotations for the corresponding generated samples. 
% We propose integrating downstream task models with the controllable generative data engine to ensure steerable and optimized data generation (consumption?).
% This is in contrast from the traditional paradigm of human-prior based data generation, wherein data distribution is pre-decided for solving the specific task.
% Task-wise, similar to the DataComp paper from LAION, but we are building an active learning framework to achieve it instead of relying on crowd-source human effort to find the best task\&model-specific data generation/composition.
Our experiments show competitive performance against state-of-the-art models using only generated synthetic data, demonstrating potential for solving downstream tasks. Project page: \href{https://synth-forge.github.io}{https://synth-forge.github.io}
% We shall release of our synthetic dataset, pretrained models, and the accompanying code-base for the community to further explore the usage of synthetic data for real-world facial analysis tasks. 
\end{abstract}

==> sec/1_intro.tex <==
\vspace{-6mm}

\section{Introduction}
\label{sec:intro}
\hf{intro bullet points for active learning dataset generator
- Controllable generative models are very powerful, they are learned from the real world distribution, hence avoid the uncanny valley issue of the traditional graphics rendering and the requirements of assets pool.
- We want to leverage controllable generative model as our synthetic data generation engine to create tons of image-gt pairs.
- However, while Controllable generative models are learned from massive data, their latent space is often too vast to obtain meaningful sample distributions for downstream task with limited generation. --> uniform sampling is not sufficient.
- We propose to forge the downstream task models together with the controllable generative data engine to make the data generation process steerable and optimized for the downstream task in an active learning way. This is in contrast from the previous paradigm of human-prior based data generation, where our generated data distribution is optimized for solving the specific discriminative task. Task-wise, similar to the DataComp paper from LAION, but we are building an active learning framework to achieve it instead of relying on crowd-source human effort to find the best task\&model-specific data generation/composition
}




The field of facial analysis encompasses a range of critical tasks, including recognition, expression analysis, and biometric authentication, each dependent on accurate face parsing tasks. As the demand for robust facial analysis systems escalates, the need for extensive and diverse datasets to train these systems becomes paramount. Recent advancements in synthesizing training data for face analysis have garnered considerable attention, pointing to a significant shift in the methodologies employed for facial recognition and analysis tasks. Traditional approaches, heavily reliant on sophisticated computer graphics pipelines \cite{fitymi,hodan2019photorealistic,hodavn2020bop}, offer the ability to render high-quality, auto-annotated facial images. However, the complexity and prohibitive cost of setting up such pipelines limit their accessibility and scalability \cite{fitymi,hodavn2020bop,hodan2019photorealistic}. Additionally, a persistent challenge with models trained on physically based rendering (PBR) synthesized imagery is the domain gap—the discrepancy between synthetic and real-world data distributions—which necessitates elaborate domain adaptation techniques to achieve practical utility.

On the other hand, the emergence of advanced generative models promises a new horizon in the generation of photo-realistic human faces. However their potential for downstream face analysis tasks is yet to be fully harnessed, primarily due to the difficulty in obtaining controllable annotations for the generated images \cite{dadnet++}. Especially in the realm of multi-task learning (MTL), the availability of dense, multi-modal supervision could enhance the efficacy of training significantly. Synthetic data is particularly well-suited for providing such comprehensive supervision for computer vision tasks as has been seen in the community \cite{fitymi,Kar_2019_ICCV,varol17_surreal,gomez2019large}, however yet remains under-explored in the facial analysis domain.

The objective of this research is to construct a multi-task facial analysis model trained on synthetic images generated by a 3DMM-controllable generative model, complemented by a technique for deriving soft annotations conducive to training tasks. To address the inherent challenges, we introduce three key insights: (i) the utilization of a generative model for the synthesis of high-quality facial images, alongside 3DMMs for extracting 3D-aware annotations, (ii) the employment of this exclusively synthesized and annotated dataset for training a robust multi-task model capable of predicting keypoints (kp), segmentation (seg), and depth modalities, and (iii) the adoption of a label fine-tuning strategy aimed at enhancing the predictions of our synthetically trained network, ensuring its adaptability to real-world datasets \cite{CelebAMask-HQ,liu2020new,karras2019style,sagonas2013300,richter2016playing}. Although the label fine-tuning strategy enhances the model's performance for evaluation purposes on existing datasets, it is primarily an evaluative/regulative step. The multi-task model, as trained exclusively with synthetic data, demonstrates strong performance on real-world data directly, underscoring its practical viability and the effectiveness of our pipeline.

A schematic of our method for obtaining multi-modal annotations is depicted in figure \ref{fig:overall_process}, along with image samples of the generated data in figure \ref{fig:banner} showcasing the practical outcomes of our proposed pipeline. The key contributions in the proposed work are as follows:

\begin{itemize}
    \item \textbf{Annotated Data Generation in a 3D-aware pipeline}: Our approach includes the extraction of soft semantic and spatial labels, leveraging sophisticated 3DMM-controllable generative model. The annotations encompass a range of facial features, providing dense, multi-modal supervision for facial analysis and parsing.
    \item \textbf{Multi-Task Framework for Synthetic Data}: The synthesized dataset is used to train a multi-task model capable of accurately predicting various facial attributes, including keypoints, segmentation, and depth. This framework demonstrates the effective use of synthetic data in training complex, multi-faceted models.
    \item \textbf{Label Fine-tuning for Real-world Adaptation}: A label fine-tuning strategy incorporating cross-task information is introduced to enhance the model’s adaptability to real-world datasets. This strategy ensures that the model, though trained on synthetic data, is capable of performing effectively on real-world images.
\end{itemize}

Our work significantly contributes to overcoming the challenges associated with the domain gap between synthetic and real-world data, demonstrating that a model trained on synthetic images can successfully be applied to real-world scenarios for face parsing and analysis. The methodology and resulting model have wide-ranging implications for the field of facial analysis, offering a scalable, cost-effective alternative to traditional data collection and annotation methods.




% \begin{figure}[h]
%   \centering
%   \begin{subfigure}{0.68\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{An example of a subfigure.}
%     \label{fig:short-a}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.28\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{Another example of a subfigure.}
%     \label{fig:short-b}
%   \end{subfigure}
%   \caption{Example of a short caption, which should be centered.}
%   \label{fig:short}
% \end{figure}



==> sec/1_intro2.tex <==
\vspace{-6mm}
\section{Introduction}
\label{sec:intro}

% Intro to facial analysis


% The field of facial analysis encompasses a range of critical tasks, including recognition, expression analysis, and biometric authentication, each dependent on accurate face parsing. As the demand for robust facial analysis systems escalates, the need for extensive and diverse datasets to train these systems becomes paramount. Traditional data collection and labeling methods are not only time-consuming and costly but also susceptible to human bias and errors. An exponential rise in data demand, fueled by the digital transformation across industries, has incited the need for innovative and efficient data acquisition techniques. Recent advancements in synthesizing training data for face analysis have garnered considerable attention, pointing to a significant shift in the methodologies employed for training facial recognition and analysis models. Unlike traditional data, which relies on real-world occurrences for collection, synthetic data is algorithmically generated, offering a plethora of advantages in terms of cost, scalability, and accuracy.

% Traditional approaches, heavily reliant on sophisticated computer graphics pipelines \cite{fitymi,hodan2019photorealistic,hodavn2020bop}, offer the ability to render high-quality, auto-annotated facial images. However, the complexity and prohibitive cost of setting up such pipelines limit their accessibility and scalability \cite{fitymi,hodavn2020bop,hodan2019photorealistic}. Additionally, a persistent challenge with models trained on physically based rendering (PBR) synthesized imagery is the domain gap — the discrepancy between synthetic and real-world data distributions — which necessitates elaborate domain adaptation techniques to achieve practical utility.

% In contrast, the emergence of advanced generative models promises a new horizon in the generation of photorealistic human faces. These models facilitate a novel form of active learning to optimize the synthetic data generation for downstream tasks. Initially, the generative model produces a set of training data, which is then used to train the downstream tasks. The performance of these tasks on validation data informs the adjustment of the generative model's latent parameters, guiding the model to generate new data that targets the downstream model's weaknesses. This method of using performance-driven parameter adjustment and selective data generation represents a strategic implementation of active learning, aiming to steer the data generation process to enhance downstream task efficacy significantly.

% The objective of this research is to demonstrate the effectiveness of this active learning approach in synthesizing training data that directly addresses the needs of downstream tasks. We introduce three key insights: (i) the utilization of a generative model for the synthesis of high-quality facial images, alongside 3DMMs for extracting 3D-aware annotations, (ii) the employment of exclusively synthesized and annotated datasets for training a robust multi-task model capable of predicting keypoints (kp), segmentation (seg), and depth modalities, and (iii) the strategic sampling of the generative distribution for representative samples aimed at improving the performance of the downstream model. As the annotation schema obtained from the generative model differs from those followed in existing benchmark datasets, we adopt a label fine-tuning strategy aimed at enhancing the predictions of our synthetically trained network to match those of real-world datasets \cite{CelebAMask-HQ,liu2020new,karras2019style,sagonas2013300,richter2016playing}. Although primarily evaluative, this strategy underscores the practical viability and effectiveness of our pipeline.

% Generative models, through this innovative active learning approach, show potential in overcoming the domain gap between synthetic and real-world data while providing a scalable and cost-effective alternative to traditional data collection and annotation methods for facial analysis. This approach not only reduces the cost of data acquisition but also ensures that the generated data is optimally beneficial for the intended facial analysis tasks. In conclusion, we demonstrate that models trained on controllably generated synthetic data perform comparably to existing state-of-the-art on various facial analysis benchmarks, showcasing the efficacy of our method.





The field of facial analysis encompasses a range of critical tasks, including recognition, expression analysis, and biometric authentication, each dependent on accurate face parsing tasks.
As the demand for robust facial analysis systems escalates, the need for extensive and diverse datasets to train these systems becomes paramount.
Traditional data collection and labeling methods are not only time-consuming and costly but also susceptible to human bias and errors.
An exponential rise in data demand, fueled by the digital transformation across industries, has incited the need for innovative and efficient data acquisition techniques.
Recent advancements in synthesizing training data for face analysis have garnered considerable attention, pointing to a significant shift in the methodologies employed for training facial recognition and analysis models.
Unlike traditional data, which relies on real-world occurrences for collection, synthetic data is algorithmically generated, offering a plethora of advantages in terms of cost, scalability, and accuracy.

Traditional approaches, heavily reliant on sophisticated computer graphics pipelines \cite{fitymi,hodan2019photorealistic,hodavn2020bop}, offer the ability to render high-quality, auto-annotated facial images.
However, the complexity and prohibitive cost of setting up such pipelines limit their accessibility and scalability \cite{fitymi,hodavn2020bop,hodan2019photorealistic}. 
Additionally, a persistent challenge with models trained on physically based rendering (PBR) synthesized imagery is the domain gap — the discrepancy between synthetic and real-world data distributions — which necessitates elaborate domain adaptation techniques to achieve practical utility.

% our approach vs deca based!? -- predictive model to get annotation

In contrast, the emergence of advanced generative models promises a new horizon in the generation of photo-realistic human faces.
However, their potential for downstream face analysis tasks is yet to be fully harnessed, primarily due to the difficulty in obtaining 3D consistent annotations for the generated images \cite{dadnet++}. 
% The availability of dense, multi-modal supervision could enhance the efficacy of training significantly. 
Synthetic data obtained from generative models is particularly well-suited for providing such comprehensive supervision for computer vision tasks as has been seen in the community \cite{fitymi,Kar_2019_ICCV,varol17_surreal,gomez2019large}, however yet remains under-explored in the facial analysis domain with 3D consistent annotations for the corresponding generated data.
Controllable generative models are usually trained on real data, and are therefore capable of generating realistic data with minimal or no domain gap.
However, the space spanned by the latent control variables of these models are generally too vast to obtain meaningful samples.
Uniformly sampling the latent space for data generation would result in samples that might not represent the distribution required to meaningfully train for a downstream task, and often provide redundant information that contributes towards scaling the dataset size without significant enhancement to task performance.


The objective of this research is to mitigate the shortcomings related to the use of controllable generative models for synthetic dataset curation, towards training downstream tasks more efficiently.
To address the inherent challenges, we introduce two key insights: (i) the utilization of a generative model for the synthesis of high-quality facial images, alongside 3DMMs for extracting 3D-aware annotations, and (ii) the employment of this exclusively synthesized and annotated dataset for training a robust multi-task model capable of predicting keypoints (kp), semantic segmentation (seg), and depth modalities
% , and (iii) an active steerable sampling of the generative model based on downstream task guided latent parameter distribution for representative samples aimed at improving the performance of the downstream model.
As the annotation schema obtained from the generative model differ from those followed in the existing benchmark datasets, we adopt a label fine-tuning strategy.
Label finetuning is aimed at enhancing the predictions of our synthetically trained network to match those of the real-world datasets \cite{CelebAMask-HQ,liu2020new,karras2019style,sagonas2013300,richter2016playing}.
Although the label fine-tuning strategy enhances the model's performance for evaluation purposes on existing datasets, it is primarily an evaluative/regulative step.
The downstream models, as trained exclusively with synthetic data, demonstrate strong performance on real-world data directly, underscoring its practical viability and the effectiveness of our pipeline.

A schematic of our method for obtaining multi-modal annotations is depicted in figure \ref{fig:overall_process}, along with image samples of the generated data in figure \ref{fig:banner} showcasing the practical outcomes of our proposed pipeline. The key contributions in the proposed work are as follows:
% \begin{itemize}
%     \item \textbf{Annotated Data Generation in a 3D-aware pipeline}: Extraction of soft semantic and spatial labels, leveraging 3DMM-controllable generative model. The annotations encompass a range of facial features, providing dense, multi-modal supervision for facial analysis and parsing.
%     \item \textbf{Multi-Task Framework for Synthetic Data}: The synthesized dataset is used to train a multi-task model capable of accurately predicting various facial attributes, including keypoints, segmentation, and depth.
%     This framework demonstrates the effective use of synthetic data in training complex, multi-faceted models.
%     \item \textbf{Sample Efficient Data Generation}: The downstream task is used to steer the data generation.
%     To ensure efficient data generation we actively generate the data using the latent sampled from the distribution where the downstream models suffers in performance.
% \end{itemize}

\begin{itemize}
    \item \textbf{Annotated Data Generation in a 3D-aware pipeline}: Utilizes a 3DMM-controllable generative model to extract soft semantic and spatial labels across a comprehensive range of facial features, providing dense, multi-modal supervision essential for detailed facial analysis and parsing.
    \item \textbf{Multi-Task Framework for Synthetic Data}: Employs a synthesized dataset to train a robust multi-task model that accurately predicts various facial attributes such as keypoints, segmentation, and depth, showcasing the potency of synthetic data in enhancing complex model training.
    % \item \textbf{Active Sampling in Data Generation}: Implements an active sampling approach where data generation is dynamically adjusted based on the performance feedback from the downstream tasks. This strategy optimizes the sampling of latent space to preferentially generate and utilize data that addresses the current shortcomings of the model, thereby increasing the efficiency and relevance of the training process.
\end{itemize}


Generative models show potential in overcoming the domain gap between synthetic and real-world data while providing a scalable and cost-effective alternative to traditional data collection and annotation methods for facial analysis.
The cost of acquiring the data from these generative models can be reduced further by efficiently sampling the latent space for the data generation process guided by the down-stream tasks.
In conclusion, we show that models trained on the controllable generative synthetic data are on par with the existing state-of-the-art on various facial analysis benchmarks. The project page is available at \href{https://synth-forge.github.io}{https://synth-forge.github.io} highlighting the links to additional resources, released dataset and code for reproducability.



% -------------- OLD ------------------- %
% By generating a corpus of data with variations across appearance, pose, and expressions, we intend to train models for tasks such as face parsing, landmark localization, and depth using exclusively our synthetic data.
% This approach shows potential in overcoming the domain gap between synthetic and real-world data while providing a scalable and cost-effective alternative to traditional data collection and annotation methods for facial analysis.
% With the efficent




% The focus of our research is to leverage generative models with an inherent parametric model for achieving 3D consistent annotations.
% We aim to extract soft semantic and spatial labels using a 3DMM-controllable generative model, Next3D \cite{next3d}.
% By generating a corpus of data with variations across appearance, pose, and expressions, we intend to train models for tasks such as face parsing, landmark localization, and depth using exclusively our synthetic data.
% This approach shows potential in overcoming the domain gap between synthetic and real-world data while providing a scalable and cost-effective alternative to traditional data collection and annotation methods for facial analysis.

% In conclusion, synthetic data holds immense potential to revolutionize the realm of machine learning.
% It offers a feasible solution to the escalating demand for data, circumvents the limitations of traditional approaches, and effectively utilizes the potential of generative models.
% Our research aims to demonstrate the efficacy of models trained on synthetic data, presenting a viable solution to real-world problems, thus heralding a new era in machine learning where manual labeling becomes redundant.



% The objective of this research is to construct a multi-task facial analysis model trained on synthetic images generated by a 3DMM-controllable generative model, complemented by a technique for deriving soft annotations conducive to training tasks. To address the inherent challenges, we introduce three key insights: (i) the utilization of a generative model for the synthesis of high-quality facial images, alongside 3DMMs for extracting 3D-aware annotations, (ii) the employment of this exclusively synthesized and annotated dataset for training a robust multi-task model capable of predicting keypoints (kp), segmentation (seg), and depth modalities, and (iii) the adoption of a label fine-tuning strategy aimed at enhancing the predictions of our synthetically trained network, ensuring its adaptability to real-world datasets \cite{CelebAMask-HQ,liu2020new,karras2019style,sagonas2013300,richter2016playing}. Although the label fine-tuning strategy enhances the model's performance for evaluation purposes on existing datasets, it is primarily an evaluative/regulative step. The multi-task model, as trained exclusively with synthetic data, demonstrates strong performance on real-world data directly, underscoring its practical viability and the effectiveness of our pipeline.

% A schematic of our method for obtaining multi-modal annotations is depicted in figure \ref{fig:overall_process}, along with image samples of the generated data in figure \ref{fig:banner} showcasing the practical outcomes of our proposed pipeline. The key contributions in the proposed work are as follows:

% \begin{itemize}
%     \item \textbf{Annotated Data Generation in a 3D-aware pipeline}: Our approach includes the extraction of soft semantic and spatial labels, leveraging sophisticated 3DMM-controllable generative model. The annotations encompass a range of facial features, providing dense, multi-modal supervision for facial analysis and parsing.
%     \item \textbf{Multi-Task Framework for Synthetic Data}: The synthesized dataset is used to train a multi-task model capable of accurately predicting various facial attributes, including keypoints, segmentation, and depth. This framework demonstrates the effective use of synthetic data in training complex, multi-faceted models.
%     \item \textbf{Label Fine-tuning for Real-world Adaptation}: A label fine-tuning strategy incorporating cross-task information is introduced to enhance the model’s adaptability to real-world datasets. This strategy ensures that the model, though trained on synthetic data, is capable of performing effectively on real-world images.
% \end{itemize}

% Our work significantly contributes to overcoming the challenges associated with the domain gap between synthetic and real-world data, demonstrating that a model trained on synthetic images can successfully be applied to real-world scenarios for face parsing and analysis.
% The methodology and resulting model have wide-ranging implications for the field of facial analysis, offering a scalable, cost-effective alternative to traditional data collection and annotation methods.



==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.




%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/method.tex <==
% \begin{figure*}[t]
%   \centering
%   \includegraphics[width=0.98\linewidth]{sec/images/SynthForge.png}
%   \caption{Overview of the process}
%   \label{fig:banner}
% \end{figure*}

\section{Method}
\label{sec:method}

% Refined version starts
% The primary objective of our research is to advance the understanding of multi-task facial analysis, prioritizing the usage of synthetically generated data. We propose a generative pipeline that consists of three principal components: (A) Synthetic data generation using a 3D-aware generative model in conjunction with an annotation synthesis module, (B) Training of a multi-task synthetic backbone network, and (C) label fine-tuning on real-world labels with cross-task learning mechanisms. In the data generation phase, (A) utilizes a 3DMM-based generative model, Next3D \cite{next3D} with FLAME \cite{flame}, to produce RGB images and corresponding annotations for various facial attributes for depth, landmarks, surface normals, and segmentation masks, offering a more expedient alternative to traditional data generation techniques \cite{??}. Following this, in (B) a synthetic backbone network with task-specific heads is trained exclusively on synthetic data, incorporating self-supervision within the shared feature backbone network. The network is subsequently frozen post-training, and we refer to this as Stage-I training. For the label fine-tuning stage in (C), the pre-trained network is fine-tuned using real images and labels, where each task's predictions are adjusted via independent label fine-tuning networks to fit the real data distribution. During this process, a cross-task loss is applied to maintain consistency among tasks, while still allowing the final networks to be independently operational after training. This comprehensive approach is designed to enhance the accuracy and generalizability of facial analysis across multiple tasks.

% The primary objective of our research is to advance the understanding of multi-task facial analysis, prioritizing the usage of synthetically generated data.
% We propose a generative pipeline that consists of three principal components: (A) Synthetic data generation using a 3D-aware generative model in conjunction with an annotation synthesis module, (B) Training of a multi-task synthetic backbone network, and (C) label fine-tuning on real-world labels with cross-task learning mechanisms.
% In this work we show that using dense supervision from different modalities  result in rich and expressive feature representations. 
% \vspace{-4mm}
% \paragraph{Data generation (A)} utilizes a 3DMM-based generative model, Next3D \cite{next3d}.
% Next3D uses FLAME \cite{flame} as the parametric head model to control the shape and expressions of the generated images.
% Leveraging the head mesh from FLAME, we obtain the corresponding annotations for various facial attributes like depth, facial landmarks and semantic segmentation for different facial features.
% % , to produce RGB images and corresponding annotations for various facial attributes for depth, landmarks, surface normals, and segmentation masks, offering a more expedient alternative to traditional data generation techniques \cite{??}.
% We describe the process in more detail in \ref{compA}. 
% \vspace{-4mm}
% \paragraph{Synthetic Backbone (B)} Following (A), in the next component, a synthetic backbone network with task-specific heads is trained exclusively on synthetic data, incorporating self-supervision within the shared feature backbone network. The network is subsequently frozen post-training, and we refer to this as Stage-I training and highlight the details in \ref{compB}.
% \vspace{-4mm}
% \paragraph{Label Finetuning (C)} For the label fine-tuning stage, the pre-trained network is fine-tuned using real images and labels, where each task's predictions are adjusted via independent label fine-tuning networks to fit the real data distribution, as discussed in \ref{compC}. During this process, a cross-task loss is applied to maintain consistency among tasks (as explained in \ref{compC1}), while still allowing the final networks to be independently operational after training. This comprehensive approach is designed to enhance the accuracy and generalizability of facial analysis across multiple tasks.
Our research aims to enhance multi-task facial analysis, with a focus on synthetic data. We introduce a three-component generative pipeline: (A) Synthetic data generation employing a 3D-aware generative model with an annotation module, (B) Training a multi-task network on synthetic data, and (C) Real-world label fine-tuning for evaluation on standard real-world benchmarks. In \textbf{Data Generation (A)}, detailed in \ref{compA}, we use Next3D \cite{next3d} and FLAME \cite{flame} to generate images and annotations for facial attributes. \textbf{Synthetic Backbone (B)} involves training a network with self-supervised learning, which is later frozen for Stage-II training (see \ref{compB}). \textbf{Label Finetuning (C)}, as elaborated in \ref{compC}, fine-tunes this network prediction head on real images, fine-tuning each task's predictions for real-world application. This approach seeks to boost the accuracy and adaptability of facial analysis tasks.

\subsection{Data Generation Pipeline}
\label{compA}

We incorporate Next3D \cite{next3d} as the 3D-aware generative model which uses FLAME as the parametric head model (3DMM), allowing a disentangled control of the facial geometry and expression in the generated image. The generative approach in Next3D models dynamic and static components with two independent tri-plane branches. The first branch is a generative texture-rasterized tri-plane which operates on a view-dependent synthesized texture map from a StyleGAN2 \cite{stylegan2} network. The inputs are a set of randomly sampled latent vector $z \sim \mathcal{N}(0, I)$ and the camera parameters for the synthesized view $c \in \mathbb{R}^{1\times25}$, where $c = K \cdot [R | t]$ represents the camera intrinsic and extrinsic parameters. The generated textures are applied to a deformed FLAME head mesh which is parameterized by the shape, expression, and pose parameters denoted as $\beta$, $\psi$, and $\theta$ respectively. The second branch models the static components into a tri-plane feature map following the method proposed in EG3D \cite{eg3d}. The tri-plane features from both the branches are fused through a neural blending module and used for neural volume rendering, followed by an image super-resolution module to generate realistic face images, $\mathcal{I}^{synth} \in \mathbb{R}^{512 \times 512 \times 3}$.

\begin{figure}[h]
    \centering
    \begin{subfigure}{0.25\columnwidth}
        \includegraphics[width=\columnwidth]{sec/images/flame-tex.png}
        \caption{Flame texture}
        \label{fig:texture}
    \end{subfigure}
    \begin{subfigure}{0.25\columnwidth}
        \includegraphics[width=\columnwidth]{sec/images/flame-tex-on-head.png}
        \caption{Flame texture on head}
        \label{fig:texture_head}
    \end{subfigure}
    \caption{UV Texture map for the FLAME head model showing semantic labels which are used to generate the segmentation annotations for our proposed data generation pipeline. These segmentation masks can be updated through the UV map to adapt to finer or coarser level of semantic information.}
    \label{fig:flame_seg}
\end{figure}

% In our proposed pipeline, the annotations for the generated images stem from two components: from the neural volume rendering pipeline of Next3D, and transformed annotations from the deformed FLAME mesh. We prepare a UV map for the FLAME head model to assign semantic colors to different parts of the head, as shown in fig. \ref{fig:flame_seg} along with the ground truth 68 facial landmarks in the 3D space. Using the camera parameters from the generative model, we project the 3D landmarks in the camera space, closely following all transformations performed in Next3D to get final 3D and 2D landmarks for the generated image. Similarly, we render the head mesh with the segmentation texture map to obtain the ground truth semantic segmentation map corresponding to the generated image. This process is contained in the Annotation module as shown in fig. \ref{fig:overall_process} (A). However, we observe some degree of misalignment in the projected data from the FLAME mesh onto the generated image owing to the multiple generative modules in the Next3D pipeline. Towards the rectification and alignment of the generated annotations, we utilise an \textit{alignment process} for the FLAME mesh which optimizes the consistency between the 3D mesh points and neural densities from the Next3D rendering module. More details and exploration about the \textit{alignment process} discussed in the Supplementary material. The depth map for the generated images is extracted during the neural rendering phase through the method proposed in NeRF \cite{nerf}. We note that the generated depth is always consistent with the generated rgb image since they are rendered through the same pipeline. Through this proposed pipeline, we are able to generate large volume of annotated data which exhibits high diversity and allows fine-grained control so as to facilitate better training in the next stage.
In our pipeline, annotations derive from Next3D's neural rendering and FLAME mesh transformations. Semantic segmentation and 68 3D landmarks from FLAME mesh's ground truth are projected onto generated images, utilizing camera parameters to align with Next3D's transformations, resulting in accurate 3D and 2D landmark representations as depicted in fig. \ref{fig:flame_seg} and fig. \ref{fig:overall_process} (A). Minor misalignments exist in the transformation process due to the non-linear transformations through the StyleGAN modules in the Next3D pipeline. Towards the rectification and alignment of the generated annotations, we utilise an \textit{alignment process} for the FLAME mesh which optimizes the consistency between the 3D mesh points and neural densities from the Next3D rendering module. More details and exploration about the \textit{alignment process} are discussed in the Supplementary material. Depth maps are consistently aligned with RGB images already, owing to volumetric rendering based on NeRF\cite{nerf}. This approach enables the creation of a diverse, large-scale annotated dataset, enhancing the training efficiency for subsequent stages.
    
\subsection{Multi-Task Synthetic Backbone (Stage I)}
\label{compB}

In \textit{Stage I}, we train a multi-task model on the synthetically generated data. This process is guided by a training regimen that capitalizes on the dense multi-task annotations provided by our data generation pipeline.
\vspace{-3mm}
\paragraph{Model Formulation:} Following common multi-task learning paradigms \cite{vandenhende2021multi,liu2019end}, the pipeline starts with the input image $x_s \in \mathbb{R}^{3 \times H \times W}$, representing the synthetically generated image $\mathcal{I}^{synth}$ in this case. This image undergoes initial processing through a feature encoder block $\mathcal{E}: \mathbb{R}^{3 \times H \times W} \to \mathbb{R}^{C \times H \times W}$, to generate the feature map $f_s = \mathcal{E}(x_s) \in \mathbb{R}^{C \times H \times W}$, where $C$ represents the number of feature channels, is the basis for further task-specific processing. Each task's processing is handled by individual task heads $\phi^{t_i}:\mathbb{R}^{C \times H \times W} \to \mathbb{R}^{C' \times H' \times W'}$. For our tasks, these heads are $\phi^{seg}$, $\phi^{depth}$, and $\phi^{kp}$, with their corresponding predictions denoted as $\hat{y}^{t_i}_s = \phi^{t_i}(f_s)$.
\vspace{-3mm}
\paragraph{Training Losses:} The training for each task utilizes specific loss functions: L1-norm loss for depth estimation ($\mathcal{L}^{depth}_s$), cross-entropy loss for semantic segmentation ($\mathcal{L}^{seg}_s$), and L2-norm loss for keypoint estimation ($\mathcal{L}^{kp}_s$). The overall task loss is defined as:
\vspace{-2mm}
\begin{equation}
    \mathcal{L}_s^{task} = \frac{1}{N} \sum\limits_{n=0}^N \sum\limits_{t_i \in \mathcal{T}} \lambda_{s,n}^{t_i} \mathcal{L}_s^{t_i}(\hat{y}^{t_i}_{s,n}, y^{t_i}_{s,n})
    \label{eq:task_loss}
\end{equation}
Here, $N$ is the number of samples, $\mathcal{T} \in \{seg, depth, kp\}$ represents the set of tasks, $\lambda_{s,n}^{t_i}$ is the loss weight for task $t_i$, and $y^{t_i}_{s,n}$ is the ground truth label for the task. Additionally, to enhance feature representation in the backbone network, we incorporate a self-supervised loss term,  based on an affine transformation $\epsilon$ applicable to both the input and the intermediate feature. The SSL loss term is formulated as:
\vspace{-2mm}
\begin{equation}
    \mathcal{L}^{SSL}_s = \frac{1}{N} \sum\limits_{n=0}^N ||\mathcal{E}(\epsilon(x_{s,n})) - \epsilon(\mathcal{E}(x_{s,n}))||_{_2}
\end{equation}
% \vspace{-2mm}
Upon completion of the training, we freeze the weights of the multi-task synthetic backbone network for use in the next stage. The network in its frozen state is denoted as $\mathcal{M}$, and its predictions are $\hat{y}^{seg}_s$, $\hat{y}^{depth}_s$, and $\hat{y}^{kp}_s$ for the respective tasks. %One of the primary motivations behind this network design is the generation of rich and robust feature representations of the data, which are crucial for effective multi-task learning.

% Refined version ends here

\subsection{Multi-Task Label Fine-tuning (Stage II)}
\label{compC}

\textit{Stage II} of our methodology focuses on label fine-tuning, a crucial process for adapting the multi-task network's predictions to various real-world datasets for fair evaluations. This stage utilizes the network trained in Stage I and fine-tunes its predictions to align with real-dataset annotations. The input to the pre-trained multi-task synthetic backbone network, denoted as $\mathcal{M}$, is $x_r \in \mathbb{R}^{3 \times H \times W} \in \mathcal{I}^{real}$, from the real-world dataset. Processing this input through $\mathcal{M}$, we obtain predictions for segmentation, depth, keypoints, and the intermediate feature map,  $(\hat{y}^{seg}_s, \hat{y}^{depth}_s, \hat{y}^{kp}_s, f_s) = \mathcal{M}(x_r)$.

\paragraph{Task-Specific Label Fine-Tuning Networks:} For each task $t_i \in \mathcal{T}$, we construct specific label fine-tuning networks, $\phi^{t_i}_L$, such as $\phi^{seg}_L$, $\phi^{depth}_L$, and $\phi^{kp}_L$, based on the tasks available in the real-world dataset. The predictions from these networks are formulated as $\hat{y}_r^{t_i} = \phi^{t_i}_L(\hat{y}_s^{t_i}, f_s)$, for each task $t_i \in \mathcal{T}$. The inclusion of the intermediate feature map $f_s$ in the fine-tuning process is optional and subject to exploration in our ablation studies. This approach is designed to account for the label disparity between synthetic and real annotations, accommodating attributes like hair and accessories that may not be present in the generated data but are found in real-world datasets.

The training of stage II follows a similar routine as in Stage I for loss metrics. The implementation of this label fine-tuning stage significantly enhances the model's versatility and utility across diverse datasets. This approach not only aligns the model's predictions with real-world data but also ensures that the model retains its robustness and accuracy, thereby elevating its overall performance in practical applications.


% \subsection{Cross-Task Feature Learning}
% \label{compC1}
% The implementation of cross-task learning in our label fine-tuning process is driven by the goal of leveraging spatial correlations and associations shared among related tasks such as depth estimation, semantic segmentation, and keypoint estimation \cite{pmlr-v119-standley20a,fifty2021efficiently}.

% \paragraph{Conceptual Framework:} Our approach, inspired by the methodology in MTPSL \cite{mtpsl}, introduces a cross-task loss defined within a joint-task space. This space is represented as \( j \in \mathbb{R}^{C_j \times H_j \times W_j} \), where \( C_j, H_j, \) and \( W_j \) are the spatial dimensions of the features in the joint-task space. The task-specific features are all projected onto the joint-task space via a mapping network and the cross-task loss is formulated based on the cosine similarity between the projected features from all task pairs.

% \paragraph{Mapping Network and Feature Modulation:} The mapping network \( m^{t_i \to j} \) is designed for each task \( t_i \) to transform task-specific predictions into the joint-task space \( j \). Except for the input encoder block, all layers in the mapping network share the same weights across tasks.

% Given a prediction \( \hat{y}_r^{t_i} \in \mathbb{R}^{C_{t_i} \times H \times W} \) for task \( t_i \), the UNet-based encoder \cite{unet} in the mapping network transforms this into a standardized feature representation \( h_r^{t_i} \in \mathbb{R}^{C \times H_c \times W_c} \). Each task has a distinct encoder, while the rest of the mapping network is shared among tasks.

% The transformation of features in intermediate layers is modulated by an auxiliary parameter \( a_{\theta, l} \). The auxiliary parameter \( a_{\theta, l} \) is utilized to modulate the task-specific features \( h_{r,l}^{t_i} \) at the \( l^{th} \) layer in the mapping network, similar to the FiLM method \cite{film}, as follows:

% \begin{equation}
%     a_{\theta, l}^{\gamma} \odot h_{r,l}^{t_i} + a_{\theta, l}^{\beta} \to h_{r,l}^{t_i}
% \end{equation}
% where \( a_{\theta, l}^{\gamma} \) and \( a_{\theta, l}^{\beta} \) are the scaling and shift parameters for the \( l^{th} \) layer.

% \paragraph{Cross-Task Loss and Regularization}: To prevent feature collapse in the joint-task space, we incorporate a regularization term that maintains a degree of similarity with the common backbone features. The overall cross-task loss is defined as:
% % \vspace{-2mm}
% \begin{equation}
% \begin{split}
% \mathcal{L}^{ct}_r = &\frac{1}{N} \sum\limits_{(t_i,t_k) \in \mathcal{T}_{p}} \lambda_{ct} \mathrm{Cos}(m^{t_i \to j}(\hat{y}^{t_i}_r), m^{t_k \to j}(\hat{y}^{t_k}_r)) \\
% &\quad + \sum\limits_{t_i \in \mathcal{T}} \lambda_{reg} \mathrm{Cos}(f_s, m^{t_i \to j}(\hat{y}^{t_i}_r))
% \end{split}
% \end{equation}
% % \vspace{-2mm}
% Here, \( \mathcal{T}_{p} \) represents the set of task pairs \( (i,k) \), with \( i \neq k \), \( f_s \) is the intermediate feature from the frozen multi-task backbone, and \( \lambda_{reg} \) is the regularization weight.

% % The table from experiments is kept here for paper arrangement
\input{sec/tables/300w}

% \paragraph{Cross-Task Training:} Employing cross-task learning enables the network to develop richer, more interconnected representations across tasks, with auxiliary parameters informing the dependency relationships between tasks. The overall training method is defined as:

% \begin{equation}
% \min\limits_{\phi_{L}^{t_i}, a_{\theta}, m^{t_i \to j}} \mathcal{L}_r^{task} + \mathcal{L}_r^{ct}  
% \end{equation}


%  In our ablation studies, we further explore the role of cross-task learning within the multi-task synthetic backbone module \( \mathcal{M} \) and present our findings and insights in the experimental results section. This methodology not only enriches feature representation but also significantly improves the adaptability and effectiveness of the model in diverse real-world applications.

==> sec/related_works.tex <==
\section{Related Works}
\noindent
\textbf{Datasets for Facial Analysis:} 
Deep learning methods that aim at facial analysis, such as face detection \cite{li2018dsfd, deng2019retinaface} and face parsing \cite{lin2021roi, Sarkar_2023_CVPR}, require high-quality face images with reliable \& accurate task-specific annotations, e.g. facial landmarks or semantic labels.
Several datasets \cite{le2012interactive, CelebAMask-HQ, liu2020new} have been proposed in this regard, which contain tens of thousands of face images. More specifically, CelebAMask-HQ\cite{CelebAMask-HQ} contains 30,000 high-resolution face images selected from the CelebA\cite{liu2015faceattributes} dataset by following CelebA-HQ\cite{karras2017progressive}. All the images have manually annotated segmentation masks of facial attributes of 512 x 512 resolution, spread among 19 classes including all facial components and accessories. Another dataset LaPa\cite{liu2020new} comprises over 22,000 facial images showcasing a wide array of expressions, poses, and occlusions. Each image in LaPa comes with an 11-category pixel-level label map and 106 facial landmark points. 

Though such datasets seem large-scale, they are often limited in terms of scalability and diversity, along with being resource intensive, and subject to human errors through manual annotations. To bridge this gap, \cite{fitymi} proposes a computer graphics inspired PBR-based synthetic data generation pipeline, procedurally generating 100,000 synthetic faces with precise 2D landmarks and per-pixel segmentation labels, allowing for vast exploration in training large-scale models on downstream tasks and real-world label adaptation. While the dataset in \cite{fitymi} boast high-fidelity and large scale nature, it is very expensive to build such a dataset owing to the cost of design, compute, and the domain-gap arising from the inherent nature of PBR-based methods.
% 
% 
% 
% 
% 
% \begin{figure*}[t]
%   \centering
%   \includegraphics[width=0.98\linewidth]{sec/images/SynthForge.png}
%   \caption{This figure illustrates a comprehensive framework for facial analysis leveraging synthetic data. (A) involves generating a synthetic dataset using a 3D-aware generative model, with annotations derived from FLAME parameters, to (B) train a multi-task prediction module ($\mathcal{M}$) with self-supervision loss in Stage I. (C) Stage II utilizes the pre-trained module to fine-tune predictions on real-world data, enhancing cross-task consistency and improving individual task performance within a joint task space. This end-to-end approach enables efficient training and deployment of facial analysis models across varied datasets.}
%   \label{fig:overall_process}
% \end{figure*}
% 
% 
% 
% 
% 
\\
\noindent
\textbf{Generative Approaches for Face Synthesis:} The progress in generative adversarial 
 learning in the past decade \cite{isola2018imagetoimage, karras2019style} has led researchers to introduce learning-based methods for generating training data. \cite{jahanian2022generative} proposes a generative framework to enable data generation for multi-view representation learning and concludes that the representations learned using generated data outperform those learned directly from real data. In the context of face synthesis, methods like \cite{HUANG2023272} propose a bi-directional method for face editing by manipulating semantic maps. A recent trend is to condition the face generation by learning an inherent 3D prior in an unsupervised setup, proposed in EG3D\cite{eg3d}. This conditioning only helps in improving the generation quality \& view consistency, however, it doesn't provide any explicit control over the generation process, e.g. manipulating facial expressions. Recent advancements in diffusion models \cite{ho2020denoising, rombach2022highresolution} have given rise to text-driven generation of high-quality and highly diverse images, with methods like \cite{zhang2023adding} provide different types of control over the denoising process. \cite{ding2023diffusionrig} leverages the parametric head model to control facial image synthesis. The usage of the parametric head model enables control over facial expressions, head pose, and even lighting, however, it doesn't allow fine-grain control over hair, beard etc. Omniavatar\cite{xu2023omniavatar} address this issue by combining both parametric as well as neural implicit head representation, where the parametric head model allows controllable generation and implicit representation models of other details such as hair, beard, accessories etc. Another similar and recent work, Next3D\cite{next3d}, built on top of EG3D utilises a FLAME \cite{flame} mesh explicitly to generate a texture map and convert to Triplanar representation, followed by volumetric rendering similar to EG3D. Although these approaches generate highly photorealistic and diverse images, a caveat is the lack of control over generation of  dense annotations.  \cite{dadnet++} addresses this issue by using a PTI-inversion \cite{roich2022pivotal} over the StyleGAN2 \cite{stylegan2} latent space in the EG3D pipeline to generate multi-view data and 3D landmarks for further training landmark estimation task. However, the lack of further dense annotations still limits the utility of existing approaches. Through the proposed pipeline in our work, we aim to bridge the gap between synthetic data generation with control over annotations, and the ease of complexity of synthetic data generation. 
 % 
 % 
 % 
 \\
 \noindent
\textbf{ Multi-task Facial Analysis:}
While there exist datasets in the facial analysis domain with annotations for multiple tasks, the exploration in the domain of multi-task learning for face parsing and analysis is very recent. \cite{lee2021face} provide a framework to mutually learn semantic segmentation and depth information through domain translation, and also release the LaPa-D dataset. \cite{zheng2021farl} explores the domain of multi-task learning through dense pre-training on text-image pairs to learn robust representations, and then fine-tunes on face parsing, alignment, and attribute recognition.; However, The success of the approach can be attributed to the extensive pre-training on the text-image dataset, which may not be easily available on a large-scale. The work presented in \cite{zheng2022decoupled} performs a cyclic self-regularization for face parsing tasks by utilizing related tasks such as edge estimation and edge categorization. The caveat with such approaches is the requirement of dense multi-task datasets which are resource intensive to compile. Multi-task approaches using partially annotated data allow for handling of sparsely annotated datasets in a multi-task manner, such as the approach shown in \cite{mtpsl}. We follow a similar methodology towards multi-task learning with cross-task feature representations combined with the capability to generate large volumes of densely annotated synthetic data. The proposed approach towards multi-task learning allows for leveraging the relationships between tasks to extract richer feature representaions in the downstream tasks

\begin{figure*}[t]
  \centering
  \includegraphics[width=0.98\linewidth]{sec/images/SynthForge.png}
  \caption{This figure illustrates a comprehensive framework for facial analysis leveraging synthetic data. (A) involves generating a synthetic dataset using a 3D-aware generative model, with annotations derived from FLAME parameters, to (B) train a multi-task prediction module ($\mathcal{M}$) with self-supervision loss in Stage I. (C) Stage II utilizes the pre-trained module to fine-tune predictions on real-world data.}
  \label{fig:overall_process}
\end{figure*}
\vspace{-3mm}

==> sec/results.tex <==
% \input{sec/tables/300w} keeping this in method section file
% \input{sec/tables/lapa}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[t!]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lccccccccccc@{}}
\toprule
\textbf{Method}                 & \textbf{Skin}  & \textbf{Hair}  & \textbf{L-eye} & \textbf{R-eye} & \textbf{U-lip} & \textbf{I-mouth} & \textbf{L-lip} & \textbf{Nose}  & \textbf{L-brow} & \textbf{R-brow} & \textbf{Mean}  \\ \midrule
Liu et al.  \cite{liu2020new}               & 92.7  & 96.3  & 88.1  & 88.0  & 84.4  & 87.6    & 85.7  & 95.5  & 87.7   & 87.6   & 89.8  \\
Te et al. \cite{te2020edge}                 & 97.3  & 96.2  & 89.5  & 90.0  & 88.1  & 90.0    & 89.0  & 97.1  & 86.5   & 87.0   & 91.1  \\
Wood et al. \cite{fitymi}                   & 97.1  & 85.7  & 90.6  & 90.1  & 85.9  & 88.8    & 88.4  & 96.7  & 88.6   & 88.5   & \textbf{90.1}  \\
FaRL-B  \cite{zheng2021farl}                & 98.00 & 96.52 & 93.97 & 93.91 & 90.15 & 91.74 & 91.21 & 97.92 & 92.70 & 92.65 & \textbf{93.88} \\ \midrule
                       % &       &       &       &       &       &         &       &       &        &        &       \\ \midrule
RS + LF $10k$ samples                                    & 96.53 & 94.26 & 86.12 & 85.58 & 81.36 & 85.48   & 85.74 & 95.68 & 85.54  & 84.48  & 87.98 \\
DECA + LF $100k$ samples                                 & 96.36 & 93.69 & 86.20 & 86.05 & 81.89 & 84.64   & 82.74 & 95.50 & 86.61  & 85.74  & 87.94 \\
% SB + LF                                     & 93.89 & 85.40 & 81.81 & 82.48 & 78.17 & 82.38   & 80.70 & 94.18 & 78.17  & 76.96  & 83.41 \\
% SB + LF w/ $f_s$                            & 96.89 & 94.51 & 88.69 & 88.87 & 74.27 & 87.90   & 87.02 & 96.21 & 87.74  & 87.34  & 88.94 \\
% SB + LF + CT  w/ $f_s$                      & 96.72  & 94.11 & 88.47 & 88.58 & 84.23 & 87.47   & 86.59 & 96.03 & 87.59  & 87.01  & 89.68 \\
SB + LF $100k$ samples                                      & 96.80 & 94.30 & 88.60 & 88.60 & 84.43 & 87.97   & 87.13 & 96.16 & 87.64  & 88.62  & \textbf{90.03} \\ \bottomrule
\end{tabular}}
\caption{Comparison with state of the art face parsing methods on the LaPa. RS, SB and LF refer to Random Sampling, Synthetic Backbone and Label Finetuning respectively. $f_s$ are the features extracted from the feature encoder $\mathcal{E}$ trained on the synthetic data.}
\label{tab:lapa}
\end{table}


% \input{sec/tables/celeba}
% \begin{table*}[]
% \begin{tabular}{lccccccccccccccc}
% Method           & face  & nose  & glasses & le    & re    & lb    & rb    & ler   & rer   & im    & ul    & ll    & hair  & neck  & mean     \\ \hline
% Wei et al.       & 96.4  & 91.9  & 89.5    & 87.1  & 85    & 80.8  & 82.5  & 84.1  & 83.3  & 90.6  & 87.9  & 91    & 91.1  & 88.1  & 87.80714 \\
% EAGR             & 96.2  & 94    & 92.3    & 88.6  & 88.7  & 85.7  & 85.2  & 88    & 85.7  & 95    & 88.9  & 91.2  & 94.9  & 89.4  & 90.27143 \\
% AGRNet           & 96.5  & 93.9  & 91.8    & 88.7  & 89.1  & 85.5  & 85.6  & 88.1  & 88.7  & 92    & 89.1  & 91.1  & 95.2  & 89.9  & 90.37143 \\
% DML-CSR          & 95.7  & 93.9  & 92.6    & 89.4  & 89.6  & 85.5  & 85.7  & 88.3  & 88.2  & 91.8  & 87.4  & 91.0  & 94.5  & 89.6  & 90.23    \\
% FaRL-B           & 96.29 & 93.72 & 93.91   & 88.75 & 88.64 & 85.24 & 85.46 & 87.06 & 87.36 & 90.96 & 87.53 & 89.81 & 95.6  & 91.54 & 90.13    \\ \hline
% SB + LF w/ $f_s$ & 95.6  & 93    & 89.13   & 86.61 & 86.32 & 83.75 & 83.61 & 84.88 & 84.57 & 89.04 & 85.85 & 88.34 & 94.03 & 89.36 & 88.15   
% \end{tabular}
% \caption{asdasd}
% \label{tab:my-table}
% \end{table*}

\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lccccccccccccccr@{}}
\toprule
\textbf{Method}  & \textbf{Face} & \textbf{Nose} & \textbf{Glasses} & \textbf{LE} & \textbf{RE} & \textbf{LB} & \textbf{RB} & \textbf{L-ER} & \textbf{R-ER} & \textbf{IM} & \textbf{UL} & \textbf{LL} & \textbf{Hair} & \textbf{Neck} & \textbf{Mean} \\ \midrule
Wei et al. \cite{wei2019accurate}      & 96.4          & 91.9          & 89.5             & 87.1        & 85          & 80.8        & 82.5        & 84.1          & 83.3          & 90.6        & 87.9        & 91.0          & 91.1          & 88.1          & 87.80      \\
EAGR    \cite{te2020edge}         & 96.2          & 94.0            & 92.3             & 88.6        & 88.7        & 85.7        & 85.2        & 88            & 85.7          & 95.0        & 88.9        & 91.2        & 94.9          & 89.4          & 90.27      \\
AGRNet   \cite{te2021adaptive}        & 96.5          & 93.9          & 91.8             & 88.7        & 89.1        & 85.5        & 85.6        & 88.1          & 88.7          & 92          & 89.1        & 91.1        & 95.2          & 89.9          & \textbf{90.37}      \\
DML-CSR  \cite{zheng2022decoupled}         & 95.7          & 93.9          & 92.6             & 89.4        & 89.6        & 85.5        & 85.7        & 88.3          & 88.2          & 91.8        & 87.4        & 91.0        & 94.5          & 89.6          & 90.23         \\
FaRL-B   \cite{zheng2021farl}        & 96.29         & 93.72         & 93.91            & 88.75       & 88.64       & 85.24       & 85.46       & 87.06         & 87.36         & 90.96       & 87.53       & 89.81       & 95.6          & 91.54         & 90.13         \\ \midrule
SB + LF w/ $f_s$ & 95.6          & 93.0            & 89.13            & 86.61       & 86.32       & 83.75       & 83.61       & 84.88         & 84.57         & 89.04       & 85.85       & 88.34       & 94.03         & 89.36         & \textbf{88.15}         \\ \bottomrule
\end{tabular}
}
\caption{Comparison with state of the art face parsing methods on CelebAMask-HQ dataset. SB, LF, $f_s$ are explained in Table \ref{tab:lapa}. LE and RE refer to the left and right ear. LB and RB refer to the left and right eyebrows. L-ER and R-ER refer to the left and right ear and, IM, UL and LL refer to inner mouth, upper and lower lips respectively. Note that we do not evaluate on facial accessories.}
\label{tab:celeb}
\end{table*}


\section{Experiments \& Results}
\label{sec:results}
\subsection{Experiment Setup}
\paragraph{Model Architecture:} We employ the UNet \cite{unet} architecture for the multi-task synthetic backbone model $\mathcal{E}$ and also for the individual heads for the depth and face parsing heads - $\phi^{depth}$ and $\phi^{seg}$.
For predicting the facial landmarks, we make use of the a $2$ layer convolution network followed by a stacked hourglass architecture \cite{newell2016stacked} with $2$ stacks - which we denote as $\phi^{kp}$ in the text.
For label finetuning, we follow the same architecture for the respective tasks.

\paragraph{Data:} The data used to train the multi-task prediction module $\mathcal{M}$ is generated at a resolution of $512 \times 512$.
We generate a dataset of 100,000 samples with varying identities and expressions by i.i.d. sampling the FLAME shape $\beta$ and expression parameters $\psi$.
To ensure that our synthetically generated data contains images from different viewpoints, we position the camera by sampling its azimuth and elevation angles from a range of $[-\pi/4, \pi/4]$.
The field of view for the camera is sampled uniformly within a range of 12$^{\circ}$ to 27$^{\circ}$ and its distance from the subject is kept at a constant $2.7$ meters. Unlike physics-based rendering methods, our data generation pipeline takes a fraction of the time to generate photo-realistic data with annotations to be leveraged for training.
Using our data generation pipeline, it took about $7$ hours to generate a dataset of 100$k$ images with 3 different annotation modalities on a single NVIDIA V100 GPU with a batch size of $1$.


We use Next3D as the 3D aware generative model for our work which features disentangled control for facial geometry via FLAME.
However, this generative model can be replaced by any existing 3D aware generative model that has the potential to leverage the 3D facial geometry to obtain facial (or presumably other kinds of) annotations.
FLAME does not have access to the textures therefore we cannot obtain perfect annotations for certain categories like eyebrows and lips.
Therefore, we leverage FLAME's texture maps \cite{flame} to manually annotate these categories onto the UV texture map that we use for segmentation - Fig. \ref{fig:flame_seg}.

\paragraph{Training:}
During training, we include data augmentations like affine transformations, perspective warping, random flipping, blurring, random erasing, adding noise, and, varying the brightness and contrast adjustments.
The images are resized to a resolution of $256 \times 256$ for all our experiments.
The multi-task prediction module $\mathcal{M}$ during stage I, is trained entirely on the synthetically generated data.
For stage I, we use a learning rate of $1e-3$ for all our task heads ($\phi^{kp}$, $\phi^{depth}$ and $\phi^{seg}$) and $1e-4$ for the feature encoder $\mathcal{E}$.

During label-finetuning (stage II), the entire multi-task module $\mathcal{M}$ is frozen.
We pass the predictions of the output heads $\hat{y}^{t_i}_s$, optionally combining the feature maps obtained from the feature encoder $\mathcal{E}$, to their respective label-finetuning networks $\phi^{t_{i}}_L$.
The reason we pass the feature maps to the label-finetuning networks is to make the model aware of facial attributes like hair, eyebrows, and lips.
% Therefore, to compare our approach with seminal works in the same facial analysis domain, we optionally pass the feature maps from $\mathcal{E}$ to the label-finetuning networks.

The learning rate in all our experiments is annealed using a cosine decay schedule with a minimum learning rate of $1e-6$.
We use AdamW optimizer to train all our models and our experiments are implemented in PyTorch \cite{Falcon_PyTorch_Lightning_2019} and Pytorch 3D \cite{ravi2020pytorch3d}.
We use Pytorch Lightning \cite{DBLP:journals/corr/abs-1711-05101} to manage and scale our experiments.

\begin{figure*}[t!]
  \centering
  \includegraphics[width=0.98\linewidth]{sec/images/lapa_res.png}
  \caption{Qualitative results on face alignment, face parsing and depth estimation task. From left to right: a) Ground truth (GT) landmarks (blue) with predicted landmarks from SB model, b) GT landmarks (blue) with predicted SB + LF w/ $f_s$ landmarks\, c) GT face parsing, d) predicted face parsing with SB , e) predicted face parsing with SB + LF + w/ $f_s$, f) GT depth map, d) predicted depth map with SB , e) predicted depth map with SB + LF + w/ $f_s$    }
  \label{fig:lapa_res}
\end{figure*}

\subsection{Datasets}
\textbf{Facial Landmark Localization:} We evaluate our approach on the 300W dataset which is a popular landmark localization benchmark.
% 300W dataset consists of 600 unique faces for training and 689 for validataion, which is further split into two categories - common (554 images) and challenge (135 images).
% Each image contains an annotated face with $68$ facial landmarks.
We note that the 300W landmarks are different from the 68 landmarks obtained from FLAME.
The difference is primarily observed around the jawline.
% thereby introducing a difference in annotation.
% The annotated landmarks follow the facial contour of the face which is different from the 3D annotations obtained from FLAME.
% (ref Fig \ref{}?).
\\
\textbf{Face Parsing:} Face parsing involves classifying the face into different regions (like nose, eyes, lips, etc.) at a pixel level.
We showcase our method's performance on two popular face parsing benchmarks - LaPa (\textbf{La}ndmark guided face \textbf{Pa}rsing) \cite{liu2020new} and CelebAMask-HQ \cite{CelebAMask-HQ}.
The faces in LaPa dataset are segmented into $11$ semantic classes.
CelebAMask-HQ is a subset of CelebA-HQ dataset containg $30,000$ high-resolution facial images wherein each image is segmented into various categories which include facial attributes like eyes, ears, nose, mouth, hair and skin.
In addition to facial attributes, this benchmarks also provides annotations for facial accessories like earrings, necklace, hats and sunglasses.\\
\textbf{Depth: } Using the depth maps curated by \cite{lee2021face}, we qualitatively showcase the results from our approach on depth estimation.


\subsection{Results}
We evaluate our approach on two facial analysis tasks - facial landmark localization and face parsing.
We also show qualitative results of our models in predicting facial depth. 
We compare our approach with existing methods that incorporate the use of synthetic data in 2 settings: a) using the entire sample set of $100k$ images for training, and b) using a randomly sampled batch of $10k$ images.
We show the performance of our approach in contrast to the popular PBR based method \cite{fitymi}, and, using DECA \cite{deca} to infer the annotations for the images from our dataset. 

Table \ref{tab:300w} showcases results for landmark localization task on the 300W dataset using the Normalized Mean Error (NME) metric - normalized by the inter-ocular outer eye distance.
We observe that our proposed synthetic backbone (SB) outperforms the PBR based method \cite{fitymi}.
The same trend is observed after label-finetuning.
Moreover, we also note that the performance of our approach is close to the state of the art methods trained entirely on real data for landmark localization.

Table \ref{tab:lapa} compares the results of our approach with other face parsing methods on the LAPA dataset.
We note that our label-finetuned synthetic backbone is very similar in performance to the PBR based method \cite{fitymi}.
We see a sharp increase in performance of our models when provided with the features $f_s$ from our synthetic feature backbone $\mathcal{E}$.
This is primarily seen in categories which are not a part of our annotation scheme like hair or have a considerable disparity from the segmentation maps in real world datasets - like eyebrows and lips.
Table \ref{tab:celeb} showcases results for face parsing on the CelebAMask-HQ dataset. We highlight that our approach is on-par with other state-of-the-art face parsing methods on this dataset. 

Fig. \ref{fig:lapa_res} shows the qualitative results on samples from the LaPa validation set for all the modalities. Notice that the predictions from the synthetic model are aligned to the groundtruth landmarks, despite never explicitly being trained on real samples. The predictions from the finetuned model also exhibit similar performance. The face parsing maps from out SB model are able to localize and segment different parts of the face accurately. The label finetuned model shows aligned predictions to the ground-truth annotations. Finally, we highlight that the predicted depth map by the SB model is qualitatively superior compared to the ground-truth reconstructed depth provided by the LaPa-D \cite{lee2021face} dataset. Notice how SB and SB+LF are able model the depth for glasses for the third identity. We showcase more qualitative results in the supplementary material.

\section{Conclusion and Limitations}
In conclusion, our work explores the integration of generative models for synthesizing high-quality face images and addresses the challenge of controllable annotations through the use of 3D Morphable Models (3DMMs). By leveraging generative synthetic data, coupled with dense multi-modal annotations, we demonstrate the efficacy of our approach in training a multi-task model for facial analysis. Our strategy includes label fine-tuning to enhance predictions on real-world datasets, supported by a robust dense multi-modal training pipeline with cross-task consistency and self-supervised losses. Our experiments reveal competitive performance against state-of-the-art single and multi-task models. Additionally, we contribute to the research community by releasing our curated dataset, pretrained models, and codebase, encouraging further exploration of synthetic data for real-world facial analysis tasks.\\
Limitations: The segmentation from the texture pipeline of the FLAME model introduces the need for a label finetuning step as FLAME does not have access to the hair, and other features like facial accessories. Moreover, the generative model used might not be consistent with the 3d annotations provided by FLAME in extreme poses.  We discuss in detail about this misalignment in the supplementary text. 

% \subsection{Datasets}
% \subsection{MTL Results}


% \begin{table}[]
% \begin{tabular}{@{}lcccr@{}}
% \toprule
% Method           & 300W & ALFW \\ \midrule
% Approach 1       &      &      \\
% Approach 2       &      &      \\
% Approach 3       &      &      \\ \midrule
% Ours             &      &      \\
% + SSL            &      &      \\
% + Label Finetune &      &      \\ \bottomrule
% \end{tabular}
% \caption{Table for results on Keypoints to compare single task performance of proposed method with current SOTA methods}
% \end{table}

% \begin{table}[]
% \begin{tabular}{@{}lcccr@{}}
% \toprule
% Method           & LaPa & Helen \\ \midrule
% Approach 1       &      & \\
% Approach 2       &      & \\
% Approach 3       &      & \\ \midrule
% Ours             &      &\\
% + SSL            &      &\\
% + Label Finetune &      &\\ \bottomrule
% \end{tabular}
% \caption{Table for results on Segmentation to compare single task performance of proposed method with current SOTA methods}
% \end{table}

% \begin{table}[]
% \begin{tabular}{@{}lcccr@{}}
% \toprule
% Method           & LaPa-D & Helen-D \\ \midrule
% Approach 1       &      & \\
% Approach 2       &      & \\
% Approach 3       &      & \\ \midrule
% Ours             &      &\\
% + SSL            &      &\\
% + Label Finetune &      &\\ \bottomrule
% \end{tabular}
% \caption{Table for results on Depth to compare single task performance of proposed method with current SOTA methods}
% \end{table}

% \begin{table}[]
% \begin{tabular}{@{}lcccr@{}}
% \toprule
% Method           & 300W  & LaPa & LaPa-D \\ \midrule
% Keypoints + Segmentation 1       &      &      &    \\
% Keypoints + Segmentation 2       &      &      &       \\
% Ours             &      &      &      \\ \midrule
% Keypoints + Depth 1       &      &      &       \\
% Ours             &      &      &      \\ \midrule
% Segmentation + Depth 1       &      &      &      \\
% Segmentation + Depth 2       &      &      &       \\
% Ours             &      &      &       \\ \bottomrule
% \end{tabular}
% \caption{Table for results to compare two task performance of proposed method with current SOTA methods}
% \end{table}

% \begin{table}[]
% \begin{tabular}{@{}lcccr@{}}
% \toprule
% Method           & 300W & LaPa &  LaPa-D  \\ \midrule
% SOTA STL Keypoints       &       &      &       \\
% SOTA STL Segmentation       &      &      &       \\
% SOTA STL Depth       &      &      &       \\
% SOTA MTL 1      &      &      &       \\
% SOTA MTL 2      &      &      &       \\ \midrule
% Ours             &     &      &       \\ 
% +SSL             &       &      &       \\ 
% +Cross Task             &      &      &       \\
% +Label Finetune             &      &      &       \\ \bottomrule
% \end{tabular}
% \caption{Table for results to compare multi-task learning performance of proposed method with current SOTA methods}
% \end{table}



% \subsection{Ablation}

% \subsubsection{Backbones}
% \begin{table}[]
% \begin{tabular}{@{}lcccr@{}}
% \toprule
% Backbone           & 300W & LaPa &  LaPa-D  \\ \midrule
% UNet       &       &      &       \\
% Hourglass       &      &      &       \\
% SegFormer       &      &      &       \\ \bottomrule
% \end{tabular}
% \caption{Table for results to different backbones to compare multi-task learning performance of proposed method}
% \end{table}

% \subsubsection{Module Ablation}
% \begin{table}[]
% \begin{tabular}{@{}lcccccr@{}}
% \toprule
% SSL           & Cross Task  & Label Finetune &  300-W &  LaPa &  LaPa-D \\ \midrule
% \checkmark &      &      &      &      &   \\
% &      \checkmark &      &       &      & \\
% &      &      \checkmark &       &      & \\
% \checkmark &     \checkmark &       &    &      &    \\ 
% \checkmark &       &     \checkmark &    &      &   \\ 
% &     \checkmark  &      \checkmark &    &      &   \\ \midrule
% \checkmark &      \checkmark &      \checkmark &    &      &   \\ \bottomrule
% \end{tabular}
% \caption{Ablation results to compare multi-task learning performance of proposed method}
% \end{table}



==> sec/tables/300w.tex <==
\begin{table}[t]
\centering
\begin{tabular}{@{}lcccr@{}}
\toprule
Method                                      & Common   & Challenge  \\ \midrule
Wood et al. \cite{fitymi}                         & 5.61     & 8.43       \\
Wood et al. \cite{fitymi} + Label Adaptation      & 3.09     & 4.86       \\
FaRL-B \cite{zheng2021farl}                              & \textbf{2.50}     & 4.42       \\
STAR  \cite{star}                               & 2.52     & \textbf{4.32}       \\
DECA \cite{deca} + LF                   & 4.26     & 7.33       \\ 
DECA \cite{deca} + LF w/ $f_s$          & 3.86     & 6.40       \\
\midrule
SB                                      & 5.74     & 9.30       \\
% SB + SSL                              &          &            \\
Random Sampling $10K$ + LF              & 5.18     & 9.25       \\
Random Sampling $10K$ + LF w/ $f_s$     & 5.06     & 8.84       \\
% Active Sampling $10K$ + LF w/ $f_s$     & 4.48     & 7.73       \\
SB + LF                                 & 3.01     & 4.96       \\ 
SB + LF w/ $f_s$                        & \textbf{2.90}     & \textbf{4.74}       \\  \bottomrule
\end{tabular}
\caption{Table for results on Keypoints to compare single task performance of proposed method with current SOTA methods. SB and LF refere to Synthetic Backbone and Label finetuning respectively. $f_s$ are the features extracted from the feature encoder $\mathcal{E}$ trained on the synthetic data.}
\label{tab:300w}
\end{table}


==> sec/tables/celeba.tex <==
% \begin{table*}[]
% \begin{tabular}{lccccccccccccccc}
% Method           & face  & nose  & glasses & le    & re    & lb    & rb    & ler   & rer   & im    & ul    & ll    & hair  & neck  & mean     \\ \hline
% Wei et al.       & 96.4  & 91.9  & 89.5    & 87.1  & 85    & 80.8  & 82.5  & 84.1  & 83.3  & 90.6  & 87.9  & 91    & 91.1  & 88.1  & 87.80714 \\
% EAGR             & 96.2  & 94    & 92.3    & 88.6  & 88.7  & 85.7  & 85.2  & 88    & 85.7  & 95    & 88.9  & 91.2  & 94.9  & 89.4  & 90.27143 \\
% AGRNet           & 96.5  & 93.9  & 91.8    & 88.7  & 89.1  & 85.5  & 85.6  & 88.1  & 88.7  & 92    & 89.1  & 91.1  & 95.2  & 89.9  & 90.37143 \\
% DML-CSR          & 95.7  & 93.9  & 92.6    & 89.4  & 89.6  & 85.5  & 85.7  & 88.3  & 88.2  & 91.8  & 87.4  & 91.0  & 94.5  & 89.6  & 90.23    \\
% FaRL-B           & 96.29 & 93.72 & 93.91   & 88.75 & 88.64 & 85.24 & 85.46 & 87.06 & 87.36 & 90.96 & 87.53 & 89.81 & 95.6  & 91.54 & 90.13    \\ \hline
% SB + LF w/ $f_s$ & 95.6  & 93    & 89.13   & 86.61 & 86.32 & 83.75 & 83.61 & 84.88 & 84.57 & 89.04 & 85.85 & 88.34 & 94.03 & 89.36 & 88.15   
% \end{tabular}
% \caption{asdasd}
% \label{tab:my-table}
% \end{table*}

\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lccccccccccccccr@{}}
\toprule
\textbf{Method}  & \textbf{Face} & \textbf{Nose} & \textbf{Glasses} & \textbf{LE} & \textbf{RE} & \textbf{LB} & \textbf{RB} & \textbf{L-ER} & \textbf{R-ER} & \textbf{IM} & \textbf{UL} & \textbf{LL} & \textbf{Hair} & \textbf{Neck} & \textbf{Mean} \\ \midrule
Wei et al. \cite{wei2019accurate}      & 96.4          & 91.9          & 89.5             & 87.1        & 85          & 80.8        & 82.5        & 84.1          & 83.3          & 90.6        & 87.9        & 91.0          & 91.1          & 88.1          & 87.80      \\
EAGR    \cite{te2020edge}         & 96.2          & 94.0            & 92.3             & 88.6        & 88.7        & 85.7        & 85.2        & 88            & 85.7          & 95.0        & 88.9        & 91.2        & 94.9          & 89.4          & 90.27      \\
AGRNet   \cite{te2021adaptive}        & 96.5          & 93.9          & 91.8             & 88.7        & 89.1        & 85.5        & 85.6        & 88.1          & 88.7          & 92          & 89.1        & 91.1        & 95.2          & 89.9          & \textbf{90.37}      \\
DML-CSR  \cite{zheng2022decoupled}         & 95.7          & 93.9          & 92.6             & 89.4        & 89.6        & 85.5        & 85.7        & 88.3          & 88.2          & 91.8        & 87.4        & 91.0        & 94.5          & 89.6          & 90.23         \\
FaRL-B   \cite{zheng2021farl}        & 96.29         & 93.72         & 93.91            & 88.75       & 88.64       & 85.24       & 85.46       & 87.06         & 87.36         & 90.96       & 87.53       & 89.81       & 95.6          & 91.54         & 90.13         \\ \midrule
SB + LF w/ $f_s$ & 95.6          & 93.0            & 89.13            & 86.61       & 86.32       & 83.75       & 83.61       & 84.88         & 84.57         & 89.04       & 85.85       & 88.34       & 94.03         & 89.36         & \textbf{88.15}         \\ \bottomrule
\end{tabular}
}
\caption{Comparison with state of the art face parsing methods on CelebAMask-HQ dataset. SB, LF, $f_s$ are explained in Table \ref{tab:lapa}. LE and RE refer to the left and right ear. LB and RB refer to the left and right eyebrows. L-ER and R-ER refer to the left and right ear and, IM, UL and LL refer to inner mouth, upper and lower lips respectively. Note that we do not evaluate on facial accessories.}
\label{tab:celeb}
\end{table*}


==> sec/tables/lapa.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[t!]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lccccccccccc@{}}
\toprule
\textbf{Method}                 & \textbf{Skin}  & \textbf{Hair}  & \textbf{L-eye} & \textbf{R-eye} & \textbf{U-lip} & \textbf{I-mouth} & \textbf{L-lip} & \textbf{Nose}  & \textbf{L-brow} & \textbf{R-brow} & \textbf{Mean}  \\ \midrule
Liu et al.  \cite{liu2020new}               & 92.7  & 96.3  & 88.1  & 88.0  & 84.4  & 87.6    & 85.7  & 95.5  & 87.7   & 87.6   & 89.8  \\
Te et al. \cite{te2020edge}                 & 97.3  & 96.2  & 89.5  & 90.0  & 88.1  & 90.0    & 89.0  & 97.1  & 86.5   & 87.0   & 91.1  \\
Wood et al. \cite{fitymi}                   & 97.1  & 85.7  & 90.6  & 90.1  & 85.9  & 88.8    & 88.4  & 96.7  & 88.6   & 88.5   & \textbf{90.1}  \\
FaRL-B  \cite{zheng2021farl}                & 98.00 & 96.52 & 93.97 & 93.91 & 90.15 & 91.74 & 91.21 & 97.92 & 92.70 & 92.65 & \textbf{93.88} \\ \midrule
                       % &       &       &       &       &       &         &       &       &        &        &       \\ \midrule
RS + LF $10k$ samples                                    & 96.53 & 94.26 & 86.12 & 85.58 & 81.36 & 85.48   & 85.74 & 95.68 & 85.54  & 84.48  & 87.98 \\
DECA + LF $100k$ samples                                 & 96.36 & 93.69 & 86.20 & 86.05 & 81.89 & 84.64   & 82.74 & 95.50 & 86.61  & 85.74  & 87.94 \\
% SB + LF                                     & 93.89 & 85.40 & 81.81 & 82.48 & 78.17 & 82.38   & 80.70 & 94.18 & 78.17  & 76.96  & 83.41 \\
% SB + LF w/ $f_s$                            & 96.89 & 94.51 & 88.69 & 88.87 & 74.27 & 87.90   & 87.02 & 96.21 & 87.74  & 87.34  & 88.94 \\
% SB + LF + CT  w/ $f_s$                      & 96.72  & 94.11 & 88.47 & 88.58 & 84.23 & 87.47   & 86.59 & 96.03 & 87.59  & 87.01  & 89.68 \\
SB + LF $100k$ samples                                      & 96.80 & 94.30 & 88.60 & 88.60 & 84.43 & 87.97   & 87.13 & 96.16 & 87.64  & 88.62  & \textbf{90.03} \\ \bottomrule
\end{tabular}}
\caption{Comparison with state of the art face parsing methods on the LaPa. RS, SB and LF refer to Random Sampling, Synthetic Backbone and Label Finetuning respectively. $f_s$ are the features extracted from the feature encoder $\mathcal{E}$ trained on the synthetic data.}
\label{tab:lapa}
\end{table}
